Learning to Broadcast for Ultra-Reliable Communication with Differential Quality of Service via the Conditional Value at Risk

Broadcast/multicast communication systems are typically designed to optimize the outage rate criterion, which neglects the performance of the fraction of clients with the worst channel conditions. Targeting ultra-reliable communication scenarios, this paper takes a complementary approach by introducing the conditional value-at-risk (CVaR) rate as the expected rate of a worst-case fraction of clients. To support differential quality-of-service (QoS) levels in this class of clients, layered division multiplexing (LDM) is applied, which enables decoding at different rates. Focusing on a practical scenario in which the transmitter does not know the fading distribution, layer allocation is optimized based on a dataset sampled during deployment. The optimality gap caused by the availability of limited data is bounded via a generalization analysis, and the sample complexity is shown to increase as the designated fraction of worst-case clients decreases. Considering this theoretical result, meta-learning is introduced as a means to reduce sample complexity by leveraging data from previous deployments. Numerical experiments demonstrate that LDM improves spectral efficiency even for small datasets; that, for sufficiently large datasets, the proposed mirror-descent-based layer optimization scheme achieves a CVaR rate close to that achieved when the transmitter knows the fading distribution; and that meta-learning can significantly reduce data requirements.

==> packages_commands_theorems.tex <==

\usepackage[utf8]{inputenc} 


\usepackage[T1]{fontenc}


\usepackage{cite}


\ifCLASSINFOpdf
 \usepackage[pdftex]{graphicx}
 \graphicspath{{../pdf/}{../jpeg/}}
 \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\else
 \usepackage[dvips]{graphicx}
 \graphicspath{{../eps/}}
 \DeclareGraphicsExtensions{.eps}
\fi



\usepackage[cmex10]{amsmath}  
\DeclareMathOperator*{\argmax}{arg\,max} 
\DeclareMathOperator*{\argmin}{arg\,min} 
\usepackage{amssymb}
\interdisplaylinepenalty=2500 

\usepackage{mathtools, nccmath}
\DeclarePairedDelimiter{\nint}\lfloor\rceil

\usepackage{algorithmic}


\usepackage{array}


\usepackage{stfloats}

\usepackage{flafter}


\usepackage{url}


\usepackage{cases}

\usepackage[colorlinks = true]{hyperref}


\usepackage{tikz}
\usetikzlibrary{calc} 
\usepackage{pgfplots}
\usetikzlibrary{patterns}
\usetikzlibrary{positioning}
\usetikzlibrary{arrows.meta} 
\usetikzlibrary{shapes} 
\usetikzlibrary{shapes.geometric} 
\usetikzlibrary{fit} 



\RequirePackage{microtype}


\usepackage{xcolor}
\definecolor{TechnionBlue}{rgb}{0, 0.1765, 0.3843} 
\definecolor{OliveGreen}{rgb}{0.4, 0.62, 0.25} 


\usepackage{ifthen}



\usepackage[normalem]{ulem}


\usepackage{fontawesome}


\newcommand{\rb}[1] {\left(#1\right)}
\newcommand{\cb}[1] {\left\lbrace #1 \right\rbrace}
\newcommand{\sqb}[1] {\left[#1\right]}
\newcommand{\given}[1]{\left\lvert#1\right.}
\newcommand{\AgivenB}[2]{\left(#1\middle\vert#2\right)}
\newcommand{\condEx}[2]{\mathbb E\left[#1\middle\vert#2\right]}
\newcommand{\condExU}[3]{\mathbb E_{#1}\left[#2\middle\vert#3\right]}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\norms}[1]{\lVert#1\rVert}
\newcommand{\normm}[1]{\big\|#1\big\|}
\newcommand*{\QEDA}{\hfill\ensuremath{\blacksquare}}
\newcommand*{\nspace}[1] {
	\ifthenelse{\equal{#1}{!}}{\!}{} 
	\ifthenelse{\equal{#1}{tq}}{\kern-1em}{} 
	\ifthenelse{\equal{#1}{mq}}{\mkern-18mu}{} 
}
\newcommand*{\KL}[2]{\text{KL}\left(#1\middle\Vert#2\right)}



\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}



\DeclareMathOperator{\tr}{tr}


